A Survey on IoT Ground Sensing Systems for Early Wildfire Detection: Technologies, Challenges and Opportunities

The threat posed by wildfires or bushfires has become a severe global issue due to the increase in human activities in forested areas and the impact of climate change. Consequently, there is a surge in the development of automatic wildfire detection methods. Approaches based on long-distance imagery from satellites or watchtowers encounter limitations, such as restricted visibility, which results in delayed response times. To address and overcome these challenges, research interest has grown in the implementation of ground-based Internet of Things (IoT) sensing systems for early wildfire detection. However, research on energy consumption, detection latency, and detection accuracy of IoT sensing systems, as well as the performance of various anomaly detection algorithms when evaluated using these metrics, is lacking. Therefore, in this article, we present an overview of current IoT ground sensing systems for early wildfire detection. Camera and environmental sensing technologies suitable for early wildfire detection are discussed, as well as vision-based detection algorithms and detection algorithms for environmental sensing. Challenges related to the development and implementation of IoT ground sensing systems for early wildfire detection and the future research directions important for creating a robust detection system to combat the growing threat of wildfires worldwide are discussed.

==> Acknowledgment.tex <==
\section*{Acknowledgment}
We thank the Australian Capital Territory Emergency Services Agency and the Australian Capital Territory Parks and Conservation Service for providing support for the collection of ignition data and their support in organising prescribed burns. We thank Sam Beaver for organising the experimental burns and Jyotirao Wankhede for assisting with the experimental burns. We also thank Dr. Andrew Sullivan and the CSIRO Bushfire Behaviour and Risks team for their help in initiating the testing of the sensing modules in the Pyrotron Lab.
